Lossy compression of discrete sources via Viterbi algorithm

We present a new lossy compressor for discrete-valued sources. For coding a sequence $x^n$, the encoder starts by assigning a certain cost to each possible reconstruction sequence. It then finds the one that minimizes this cost and describes it losslessly to the decoder via a universal lossless compressor. The cost of each sequence is a linear combination of its distance from the sequence $x^n$ and a linear function of its $k^{\rm th}$ order empirical distribution. The structure of the cost function allows the encoder to employ the Viterbi algorithm to recover the minimizer of the cost. We identify a choice of the coefficients comprising the linear function of the empirical distribution used in the cost function which ensures that the algorithm universally achieves the optimum rate-distortion performance of any stationary ergodic source in the limit of large $n$, provided that $k$ diverges as $o(\log n)$. Iterative techniques for approximating the coefficients, which alleviate the computational burden of finding the optimal coefficients, are proposed and studied.

==> notations.tex <==
Let $\Xc$ and $\hat{\Xc}$ denote the source and reconstruction
alphabets respectively. Let matrix
$\mathbf{m}(y^n)\in\mathds{R}^{|\hat{\Xc}|}\times\mathds{R}^{|\hat{\Xc}|^{k}}$
represent $(k+1)^{\rm th}$ order empirical count of $y^n$
defined as
\begin{equation}\label{eq: empirical count matrix}
    m_{\b,\bb}(y^n) = \frac{1}{n-k} \left| \left\{ k+1 \leq i \leq n : y_{i-k}^{i-1} = \bb, y_i=\b  \right\} \right|.
\end{equation}
%In \eqref{eq: empirical count matrix}, and throughout we assume
%a cyclic convention whereby $y_i \triangleq y_{n+i}$ for $i
%\leq 0$.
Let $H_k (y^n)$ denote the conditional empirical
entropy of order $k$ induced by $y^n$, i.e.~
\begin{equation}\label{eq: emp cond distribution}
    H_k (y^n) = H(Y_{k+1} | Y^{k}) ,
\end{equation}
where $Y^{k+1}$ on the right hand side of (\ref{eq: emp cond
distribution}) is distributed according to
\begin{equation}\label{eq: empirical distribution}
    \P (Y^{k+1} = [\bb,\b]) = m_{\b,\bb}(y^n),
\end{equation}
where $\b\in\hat{\Xc}$, and $\bb\in\hat{\Xc}^{k}$, and
$[\bb,\b]$ represents the vector made by concatenation of $\bb$
and $\b$. We will use the same notation throughout the paper,
namely, $\b,\b',\ldots\in\hat{\Xc}$, and   $\bb, \bb',
\ldots\in\hat{\Xc}^k$. The conditional empirical entropy in
\eqref{eq: emp cond distribution} can be expressed as a
function of $\mb(y^n)$ as follows
\begin{equation}\label{eq: alternative representation of Hk}
H_k (y^n) = H_k (\mb(y^n)) :=\frac{1}{n} \sum_{\b,\bb} \mathcal{H} \left(
\mb_{\cdot,\bb}(y^n) \right) \mathbf{1}^T \mb_{\cdot,\bb}(y^n),
\end{equation}
where $\mathbf{1}$ and  $\mb_{\cdot,\bb}(y^n)$ denote the
all-ones column vector of length $|\hat{\Xc}|$, and the column
in $\mb(y^n)$ corresponding to $\bb$ respectively. For a vector
$\mathbf{v} = (v_1, \ldots , v_\ell)^T$ with non-negative
components, we let $\mathcal{H}(\mathbf{v})$ denote the entropy
of the random variable whose probability mass function (pmf) is
proportional to $\mathbf{v}$. Formally,
\begin{equation}\label{eq: single letter ent functional defined}
\mathcal{H} (\mathbf{v}) = \left\{ \begin{array}{cc}
                            \sum\limits_{i=1}^\ell \frac{v_i}{\| \mathbf{v} \|_1}  \log \frac{\| \mathbf{v} \|_1}{v_i} &  \mbox{ if }  \mathbf{v} \neq (0, \ldots , 0)^T \\
                            0 & \mbox{ if } \mathbf{v}  = (0, \ldots , 0)^T.
                          \end{array}
\right.
\end{equation}

